A quantitative model for the emergent population dynamics of the melanoma MITF rheostat

Cancer progression is driven by the ability of cells with identical driver mutations to adopt biologically distinct adaptive phenotypes. Yet the population dynamics implied by intratumour phenotypic heterogeneity is poorly understood. Melanoma is an excellent setting to study phenotype switching, in part because phenotypic identity is conferred by melanocyte inducing transcription factor (MITF) activity. Here we develop a multiscale phenotype-structured partial differential equation model for epidermal melanoma cell populations, first considering subcellular MITF and then spatially uniform and spatially heterogeneous populations. The model admits three stable long-term behaviours: slow growth with proliferative cells and non-cycling differentiated cells; faster expansion, with an invasive core; and rapid growth with oscillatory core dynamics. More broadly, the analysis highlights that phenotype reversibility by individual cells does not imply reversibility of phenotype population distributions. Hence, single-cell properties (e.g., reversibility of invasive capacity) must be extrapolated with caution to populations with coupled cell dynamics.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


